Seamless Object-Oriented Requirements

Design by Contract enables seamless software development by unifying software requirements with their implementations. In its pure form, however, Design by Contract leaves some problems with contracts' expressiveness, verifiability, and reusability open. These problems significantly reduce practical applicability of seamless development. The present article introduces seamless object-oriented requirements - a novel approach to seamless development that builds upon Design by Contract and now-available advanced program proving tools. The article explains and illustrates the new approach, concluding with a quantitative evaluation of the extent to which the approach fixes the problems of traditional contracts.

==> sections/InternalsOfTemplates.tex <==
Construction of SOORTs follows the same algorithm (\Cref{unified_solution:activities:soort_development}), which is why detailing one of them should suffice for understanding the overall idea.
The SOORTs' structure follows the philosophy of capturing as much complexity as possible, to simplify specification of concrete SOORs.
Specifying a SOOR from a SOORT consists of the following steps:
\begin{enumerate}
	\item Inheriting from the SOORT.
	\item Replacing the SOORT's formal generic parameters with the specified types.
	\item Connecting the SOORT's deferred features with the specified types' concrete features.
\end{enumerate}

From the extensibility viewpoint, the approaches to specifying SOORTs for control software and for software components differ as follows:
\begin{itemize}
	\item A SOORT for control software represents an SRP capturing a finalized behavior.
	\item A SOORT for software components is an extensible collection of related behaviors.
\end{itemize}
The following sections illustrate this difference on specific examples.

\subsection{Requirement templates for control software} \label{soort_internals:control_software}

\begin{figure}
	\centering
	\lstinputlisting[numbers=left]{response_global.e}	
	\caption[The SOORT encoding the ``global response'' SRP]{The SOORT encoding the ``Global Response'' SRP from the catalogue of Dwyer et al (\Cref{response_global}).
	Specification driver \e{verify} encodes the formal semantics of the SRP.
	String function \e{requirement_specific_output} produces the natural language representation of the SRP parameterized with the formal generic parameters' names.
	Integer function \e{time_boundary}, inherited from \e{REQUIREMENT}, specifies the default time boundary for finite verification.}
	\label{fig:global_response}
\end{figure}

\Cref{fig:global_response} depicts the Eiffel SOORT corresponding to the most frequently recurring SRP identified by Dwyer et al. -- the ``Global Response'' SRP (\Cref{response_global}).
Out of the 555 requirements analyzed by Dwyer et al., 241 were instances of this SRP \cite{DBLP:conf/icse/DwyerAC99}.
It takes the following form in LTL:
\begin{equation}
	\square (P \implies \Diamond S)
\end{equation}
where $P$ is called ``stimulus'' and $S$ is called ``response''; ``$\square$'' and ``$\Diamond$'' encode for the ``always'' and ``eventually'' temporal logic \cite{DBLP:conf/focs/Pnueli77} operators.
Line 2 in \Cref{fig:global_response} captures the string representation of the SRP, where \e{S} and \e{P} vary between requirements.
Line 3 provides a named hyperlink to a OneNote page detailing the SRP in the initial 5 notations provided by Dwyer et al. \cite{DBLP:conf/icse/DwyerAC99}.
Line 4 provides a named hyperlink to the location of the class on GitHub.
The EIS (Eiffel Information System) mechanism of EiffelStudio makes it possible to construct, maintain and follow named hyperlinks.
Lines 6-7 declare the class capturing the SRP. The declaration depends on three formal generic parameters -- \e{G}, \e{S} and \e{P}:
\begin{itemize}
	\item \e{G} stands for the specified type.
	\item \e{S} formalizes the ``S'' in the string representation.
	\item \e{P} formalizes the ``P'' in the string representation.
\end{itemize}
The S and P parameters are constrained: they must be conditions over the specified type G.
Requiring these types to be expanded allows them to have default objects; the benefits of this possibility are coming shortly.

Lines 13-28 implement the \e{verify} routine that captures the SRP's formal semantics as a specification driver.
The routine accepts a formal argument of the specified type and expresses the SRP's semantics in terms of this variable.
Lines 16-17 require the stimulus to hold through the precondition, where:
\begin{itemize}
	\item \e{p_holds} is a tag for easier debugging.
	\item \e{(\{P\}).default} returns the default object of type \e{P}.
	\item \e{holds} is a deferred Boolean function declared in class \e{CONDITION}, from which \e{P} inherits.
	\item The \e{(\{P\}).default.holds (system)} assertion requires the stimulus to hold for \e{system}, the formal parameter of \e{verify}.
\end{itemize}
Lines 19-20 initialize the timer variable declared in the parent \e{REQUIREMENT} class.
Lines 21-22 capture the response \e{S} through the loop exit condition.
Lines 23-24 modify the system's state, where:
\begin{itemize}
	\item The \e{iterate} command is implemented in the \e{REQUIREMENT} class.
	\item \e{iterate} calls deferred command \e{main} of that class and decreases the timer.
	\item \e{main} is deferred for being implemented in concrete SOORs inheriting from the SOORT.
\end{itemize}
Lines 25-26 guarantee termination of the loop through the timer used as the loop variant.
The \e{verify} routine, when called appropriately on a SOOR implementing the template, becomes a test method; this maps to the ``Verifying through testing'' activity (\Cref{unified_solution:activities:verify_through_testing}).
When submitted to AutoProof, it becomes a Hoare logic theorem capturing the requirement's correctness axiom; this maps to the ``Verifying through program proving" activity (\Cref{unified_solution:activities:verify_through_proving}).

String function \e{requirement_specific_ouput} on lines 32-35 returns the SRP-dependent natural language representation.
The \e{REQUIREMENT} class implements, among other features, string function \e{out} which, in its turn, takes the value of \e{requirement_specific_ouput} and embeds it into the SRP-independent natural language representation.
The SRP-independent part includes the name of the requirement derived from the SOOR's class name, the name of the specified type and the real-time constraint.

The \e{time_boundary} function returns the default time boundary for finite state verification.
This value comes from the \e{REQUIREMENT} ancestor class and is set to\\
\e{\{INTEGER\}.max_value}, the maximum integer avaiable on the current system.
Concrete SOORs may override this default.
The verification process will simulate up to that number of executions of \e{iterate} to observe the required response.
If the response is not observed after the last iteration, the verification process will fail.

\subsection{ADT templates for software components} \label{soort_internals:software_components}

\begin{figure}
	\centering
	\lstinputlisting[numbers=left]{binary_tree_with_inord_adt.e}	
	\caption[The SOORT encoding the binary tree with ``in order'' ADT]{The SOORT for the ADT specification of binary tree with function ``in order'' \Cref{binary_tree_with_inord_adt}).
%	The list of the template's formal generic parameters includes type \e{Q}; type \e{QS} that must specify queues of elements of \e{I} and thus conform to the \e{QUEUE_WITH_APPEND_ADT [Q, I]} type.
	It inherits specification drivers of the \e{BINARY_TREE_ADT} SOORT encoding the ADT specification of binary tree without that function.
%	The new template inherits from the parent all its definitions and axioms, adding its own: deferred definition \e{in_ord}, \e{a_11} and \e{a_12}, well-definedness axiom for \e{in_ord}.
	}
	\label{fig:binary_tree}
\end{figure}

\Cref{fig:binary_tree} depicts the SOORT capturing the Binary Tree ADT specification with the \e{in_ord} function (\Cref{binary_tree_with_inord_adt}).
The class consists of the following important parts:
\begin{itemize}
	\item Line 2 in \Cref{fig:binary_tree} provides a general description of the template.
	\item Lines 3-4 provide a hyperlink to the source of the specification in the literature.
	\item Line 5 provides a named hyperlink to the location of the class on GitHub.	
	\item Lines 7-8 declare type \e{B} intended to behave as a binary tree containing elements of \e{I}; \e{Q} stands for the queue type returned by the \e{in_ord} function.
	To show that \e{Q}, indeed, behaves as a queue of \e{I}s, the template's implementers must supply type \e{QS} conforming to the \e{QUEUE_WITH_APPEND_ADT} template applied to \e{Q} and \e{I}.
	\item Lines 13-15 reflect the fact that the current SOORT inherits the regular binary tree behavior.
	\item Lines 17-22 declare the new function, \e{in_ord} (``in order'').
	\item Lines 24-50 state the ADT axioms due to the new function.
	\item Lines 52-61 state the well-definedness axiom for the contract of \e{in_ord}.	
\end{itemize}

Unlike the SOORTs for control software (\Cref{soort_internals:control_software}), ADT SOORTs have several specification drivers for verification.
In the example on \Cref{fig:binary_tree}, the new SOORT adds two axioms, \e{a_11} and \e{a_12}, to the axioms inherited from the parent SOORT.
Because the new ADT declares another function, \e{in_ord}, these new axioms are required for completeness of the resulting ADT specification.
The \e{in_ord_well_defined} auxiliary axioms requires the contract of \e{in_ord} to be well-defined.
Well-definedness axioms apply only to verification with AutoProof: they make sure that the respective features' contracts are strong enough to maintain the equivalence classes.

To specify a SOOR stating that objects of a custom type \e{T} behave as binary trees with elements of \e{E}, convertible to queues \e{F} with elements of \e{E}:

\begin{enumerate}
	\item Inherit from the \e{BINARY_TREE_WITH_INORD_ADT} class with \e{T} for \e{B}, \e{E} for \e{I}, \e{F} for \e{Q}.
	\item For \e{QS}, provide a SOOR that specifies \e{F} as queue with elements of \e{E}.
	\item Implement the SOORT's deferred definitions in terms of the features of types \e{T}, \e{E} and \e{F}.
\end{enumerate}
To verify correctness of \e{T} against the binary tree axioms:
\begin{enumerate}
	\item Run the specification drivers with names \e{a_*} on relevant test input (that is, satisfying the specification driver's precondition) if you practice testing.
	\item If you practice program proving, submit the resulting SOOR to AutoProof.
\end{enumerate}

ADT SOORTs differ conceptually from control software SOORTs with their extensibility.
If a variation of an ADT emerges, then making the new SOORT a subclass of the original ADT's SOORT will automatically include its specification drivers.
SOORTs for control software have finer granularity: they represent finalized behavioral patterns.

